Neural Fourier Shift for Binaural Speech Rendering

We present a neural network for rendering binaural speech from given monaural audio, position, and orientation of the source. Most of the previous works have focused on synthesizing binaural speeches by conditioning the positions and orientations in the feature space of convolutional neural networks. These synthesis approaches are powerful in estimating the target binaural speeches even for in-the-wild data but are difficult to generalize for rendering the audio from out-of-distribution domains. To alleviate this, we propose Neural Fourier Shift (NFS), a novel network architecture that enables binaural speech rendering in the Fourier space. Specifically, utilizing a geometric time delay based on the distance between the source and the receiver, NFS is trained to predict the delays and scales of various early reflections. NFS is efficient in both memory and computational cost, is interpretable, and operates independently of the source domain by its design. Experimental results show that NFS performs comparable to the previous studies on the benchmark dataset, even with its 25 times lighter memory and 6 times fewer calculations.

==> tab/ood-objective.tex <==
%\begin{table*}[t]
\begin{table}[t]
    \centering
    %\setlength{\abovecaptionskip}{5pt}
    \footnotesize
    \begin{tabular}{c|c}\toprule
        \textbf{Model} &
        \textbf{Speech}
        \\\midrule
        WarpNet \cite{richard2020neural} &  2.5803
        \\
        BinauralGrad \cite{leng2022binauralgrad} & 1.8463 \\\midrule
        Ours (random scale) &  
        \\
        Ours (random shift) &  
        \\\midrule
        Ours (wo NI) &  
        \\
        \textbf{Ours (NFS)} & 3.1460
        \\\bottomrule
    \end{tabular}
    \caption{PESQ results for out-of-distribution samples.
    }
    \label{tab:objective}
\end{table}
%\end{table*}


==> tab/ood-subjective.tex <==
%\begin{table*}[t]
\begin{table}[t]
    \centering
    %\setlength{\abovecaptionskip}{5pt}
    \footnotesize
    \begin{tabular}{l|ccc}\toprule
        \textbf{Model} &
        \textbf{Singing} & \textbf{Music} & \textbf{General Noise}
        \\\midrule
        WarpNet \cite{richard2020neural} & $2.87$ {\tiny $\pm 1.08$} & $2.73$ {\tiny $\pm 1.14$} &  $2.82$ {\tiny $\pm 1.11$} 
        \\
        BinauralGrad \cite{leng2022binauralgrad} & $2.91$ {\tiny $\pm 1.07$}  & $2.84$ {\tiny $\pm 1.11$}  & $2.96$ {\tiny $\pm 0.98$} 
        \\\midrule
        \textbf{Ours (NFS)} & $2.83$ {\tiny $\pm 0.91$}  & \textbf{$2.91$ {\tiny $\pm 0.98$}}  & $2.70$ {\tiny $\pm 0.94$} 
        \\
        \quad {\tt\footnotesize wo.Shifter} & $2.49$ {\tiny $\pm 1.04$}  & $2.62$ {\tiny $\pm 1.14$}  & $2.50$ {\tiny $\pm 1.02$}
        \\
        \quad {\tt\footnotesize wo.NI} & $2.83$ {\tiny $\pm 0.91$}  & $2.78$ {\tiny $\pm 1.03$}  & $2.86$ {\tiny $\pm 0.89$}
        \\\bottomrule
    \end{tabular}
    \caption{Mean opinion score for out-of-distribution samples.
    Participants are asked to score spatialization on a Likert scale from 1 to 5.
    }
    \label{tab:ood}
\end{table}
%\end{table*}


==> tab/subjective.tex <==
%\begin{table*}[t]
\begin{table}[t]
    \centering
    %\setlength{\abovecaptionskip}{5pt}
    \footnotesize
    \begin{tabular}{c|c|cc}\toprule
        \textbf{Model} & \textbf{\# params} &
        \textbf{MOS} & \textbf{PESQ}
        \\\midrule
        WarpNet \cite{richard2020neural} & 8.59 M &  
        \\
        BinauralGrad \cite{leng2022binauralgrad} & 13.8 M & 
        \\\midrule
        Ours (wo noise injection) & 0.58 M &  
        \\
        Ours (wo shifter) & 0.31 M &  
        \\\midrule
        Ours (wo NI) & \textbf{0.xx M} &  
        \\
        \textbf{Ours (NFS)} & \textbf{0.58 M} &  
        \\\bottomrule
    \end{tabular}
    \caption{Perceptual evaluation results.
    }
    \label{tab:objective}
\end{table}
%\end{table*}

